Thin-Film Smoothed Particle Hydrodynamics Fluid

We propose a particle-based method to simulate thin-film fluid that jointly facilitates aggressive surface deformation and vigorous tangential flows. We build our dynamics model from the surface tension driven Navier-Stokes equation with the dimensionality reduced using the asymptotic lubrication theory and customize a set of differential operators based on the weakly compressible Smoothed Particle Hydrodynamics (SPH) for evolving pointset surfaces. The key insight is that the compressible nature of SPH, which is unfavorable in its typical usage, is helpful in our application to co-evolve the thickness, calculate the surface tension, and enforce the fluid incompressibility on a thin film. In this way, we are able to two-way couple the surface deformation with the in-plane flows in a physically based manner. We can simulate complex vortical swirls, fingering effects due to Rayleigh-Taylor instability, capillary waves, Newton's interference fringes, and the Marangoni effect on liberally deforming surfaces by presenting both realistic visual results and numerical validations. The particle-based nature of our system also enables it to conveniently handle topology changes and codimension transitions, allowing us to marry the thin-film simulation with a wide gamut of 3D phenomena, such as pinch-off of unstable catenoids, dripping under gravity, merging of droplets, as well as bubble rupture.

==> bo_macr.bak.tex <==
\usepackage{xcolor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Common
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newif\ifsingle
%\singletrue     % set true for single-author mode

%\ifsingle
\newcommand{\bo}[1]{\textcolor{blue}{[#1]}}
%\else
%\newcommand{\bo}[1]{\textcolor{blue}{[Bo: #1]}}
%\fi

%\ifsingle
\newcommand{\mengdi}[1]{\textcolor{red}{[#1]}}
%\else
%\newcommand{\mengdi}[1]{\textcolor{red}{[Mengdi: #1]}}
%\fi


%%%% Put authors command here
\newcommand{\wmd}[1]{\textcolor{red}{[wmd: #1]}}
\newcommand{\yitong}[1]{\textcolor{red}{[yitong: #1]}}
\newcommand{\kxx}[1]{\textcolor{red}{[kxx: #1]}}
\newcommand{\xiong}[1]{\textcolor{red}{[xiong: #1]}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Figures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% wrap figure
% file name, caption, label, width (ratio), height (inch)
% example: \WrapFig{beak.png}{This is a wrap figure.}{fig:beak}{.5}{1.5}
% placeholder example: \WrapFig{example-image}{This is a wrap figure.}{fig:beak}{.5}{1.5}
% we can also use example-image-a/b/c
\newcommand{\WrapFig}[5]
{
\begin{wrapfigure}{r}{{#4}\textwidth}
	\vspace{-.5\baselineskip}
	\centering
	\includegraphics[height={#5}in]{#1}
	\caption{#2}
	\vspace{-.25\baselineskip}
	\label{#3}
\end{wrapfigure}
}
\newcommand{\WrapFigL}[5]
{
\begin{wrapfigure}{l}{{#4}\textwidth}
	\vspace{-.5\baselineskip}
	\centering
	\includegraphics[height={#5}in]{#1}
	\caption{#2}
	\label{#3}
\end{wrapfigure}
}

%wrap figure with out caption number
%file name, caption, label, width (ratio), height (inch)
%example: \WrapFigNoNum{beak.png}{This is a wrap figure.}{fig:beak}{.5}{1.5}
\newcommand{\WrapFigNoNum}[5]
{
\begin{wrapfigure}{r}{{#4}\textwidth}
	\vspace{-.5\baselineskip}
	\centering
	\includegraphics[height={#5}in]{#1}
	\caption*{#2}
	\label{#3}
\end{wrapfigure}
}
\newcommand{\WrapFigNoNumL}[5]
{
\begin{wrapfigure}{l}{{#4}\textwidth}
	\vspace{-.5\baselineskip}
	\centering
	\includegraphics[height={#5}in]{#1}
	\caption*{#2}
	\label{#3}
\end{wrapfigure}
}

%figure on top
%file name, caption, label, width (ratio)
%example: \TopFig{beak.png}{This is a top figure.}{fig:beak}{1.}
\newcommand{\TopFig}[4]
{
\begin{figure}[t!]
	\centering
	\includegraphics[width=#4\textwidth]{#1}
	\caption{#2}
    \label{#3}	
\end{figure}
}

%figure on top
%file name, caption, label, width (ratio)
%example: \BotFig{beak.png}{This is a top figure.}{fig:beak}{1.}
\newcommand{\BotFig}[4]
{
\begin{figure}[b!]
	\centering
	\includegraphics[width=#4\textwidth]{#1}
	\caption{#2}
    \label{#3}	
\end{figure}
}


\newcommand{\HereFig}[4]
{
\begin{figure}[h!]
	\centering
	\includegraphics[width=#4\textwidth]{#1}
	\caption{#2}
    \label{#3}	
\end{figure}
}

\newcommand{\FourTeaserFig}[5]
{
\begin{teaserfigure}
    \centering
    \includegraphics[width=.24\textwidth]{#1}
    \includegraphics[width=.24\textwidth]{#2}
    \includegraphics[width=.24\textwidth]{#3}
    \includegraphics[width=.24\textwidth]{#4}
  \caption{#5}
  \label{fig:teaser}
\end{teaserfigure}
}

\newcommand{\ThreeTeaserFig}[4]
{
\begin{teaserfigure}
    \centering
    \includegraphics[width=.33\textwidth]{#1}
    \includegraphics[width=.33\textwidth]{#2}
    \includegraphics[width=.33\textwidth]{#3}
  \caption{#4}
  \label{fig:teaser}
\end{teaserfigure}
}

\newcommand{\magicfigure}[8]{
% #1 is width of the small guys
% #2 is the height of the big guy
% #3 is horizontal pad
% #4-#9 are figures
{\hfill\hbox{\includegraphics[height=#2,draft=\mydraft]{#4}\hspace{#3}\vbox to #2{\hbox{\includegraphics[width=#1,draft=\mydraft]{#5}\hspace{#3}\includegraphics[width=#1,draft=\mydraft]{#6}}\vfill\hbox{\includegraphics[width=#1,draft=\mydraft]{#7}\hspace{#3}\includegraphics[width=#1,draft=\mydraft]{#8}}}}\hfill}
%}

\newcommand{\supermagicfigure}[9]{
% #1 is width of the small guys
% #2 is the height of the big guy
% #3 is horizontal pad
% #4-#9 are figures
%\includegraphics[height=#2,draft=\mydraft]{#3}
%{\hfill\hbox{\hspace{.01in}\vbox to#2{\hbox{\includegraphics[width=#1,draft=\mydraft]{#4}\hspace{.01in}\includegraphics[width=#1,draft=\mydraft]{#5}\hspace{.01in}\includegraphics[width=#1,draft=\mydraft]{#6}}\vfill\hbox{\includegraphics[width=#1,draft=\mydraft]{#7}\hspace{.01in}\includegraphics[width=#1,draft=\mydraft]{#8}\hspace{.01in}\includegraphics[width=#1,draft=\mydraft]{#9}}}}\hfill}
{% to #2 
    \hfill
    \hbox{
        \hspace{#3}
        \vbox{
            \hbox{
                %\includegraphics[width=#1,draft=\mydraft]{#4}\hspace{#3}
                \includegraphics[width=#1,draft=\mydraft]{#5}\hspace{#3}
                \includegraphics[width=#1,draft=\mydraft]{#6}
            }
            \vfill
            \hbox{
                %\includegraphics[width=#1,draft=\mydraft]{#7}\hspace{#3}
                \includegraphics[width=#1,draft=\mydraft]{#8}\hspace{#3}
                \includegraphics[width=#1,draft=\mydraft]{#9}
            }
        }
    }
    \hfill
    }
}

%\begin{comment}
%\begin{figure*}
%\centering
%    \magicfigure{.245\textwidth}{.372\textwidth}{.03in}{figures/fishbone_img1.png}{figures/fishbone_img2.png}{figures/fishbone_img3.png}{figures/fishbone_img4.png}{figures/fishbone_img5.png}
%    \caption{Two colliding liquid jets form a fluid fishbone \protect\cite{John:2002:fishbone}. Surface tension causes the rim of the thin sheet to pinch off into many filaments and droplets.\label{fig:fishbone}}
%    \vspace{-0.2in}
%\end{figure*}
%\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Math
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bw}{\vec{w}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bj}{\mathbf{j}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% verbose and blabla
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifverbose
\verbosetrue

\ifverbose
\newcommand{\sota}{\textcolor{red}{\textbf{(SOTA)}} }
\newcommand{\howto}{\textcolor{red}{\textbf{(How to)}} }
\newcommand{\diff}{\textcolor{red}{\textbf{(Difference)}} }
\newcommand{\problem}{\textcolor{red}{\textbf{(Problem)}} }
\newcommand{\chal}{\textcolor{red}{\textbf{(Challenge)}} }
\newcommand{\expe}{\textcolor{red}{\textbf{(Expertise)}} }
\newcommand{\impo}{\textcolor{red}{\textbf{(Importance)}} }
\newcommand{\insight}{\textcolor{red}{\textbf{(Insight)}} }
\newcommand{\plan}{\textcolor{red}{\textbf{(Plan)}} }
\newcommand{\wepropose}{\textcolor{red}{\textbf{(We propose)}} }
\newcommand{\vb}[1]{\textcolor{red}{#1}}
\else
\newcommand{\sota}{}
\newcommand{\howto}{}
\newcommand{\diff}{}
\newcommand{\problem}{}
\newcommand{\chal}{}
\newcommand{\expe}{}
\newcommand{\impo}{}
\newcommand{\insight}{}
\newcommand{\plan}{}
\newcommand{\wepropose}{}
\newcommand{\vb}[1]{}
\fi

\newcommand{\bladot}{$\quad\cdot$ }
\newcommand{\bla}{\noindent\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot\bladot}
\newcommand{\blaii}{\bla \\ \bla \\}
\newcommand{\blaiii}{\bla \\ \bla \\ \bla \\}
\newcommand{\blaiv}{\blaii \blaii}
\newcommand{\blaoct}{\blaiv \blaiv}
\newcommand{\blahex}{\blaoct \blaoct}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> notes.tex <==
References:

######################################
Thin film and surface tension flow:

- Eitan Grinspun's visous sheet, filament
http://www.cs.columbia.edu/cg/pdfs/171-threads.pdf
https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.296.4654&rep=rep1&type=pdf

- Mesh-based ones:
    * Fang Da's bubble papers
    http://www.cs.columbia.edu/cg/doublebubbles/doublebubbles.pdf
    * Chris Wojtan's bubbles
    * Ryoichi Ando's bubbles
    https://sadashigeishida.bitbucket.io/hgf/hgf.pdf
    * Bo's bubbles
    sci-hub.se/10.1145/2601097.2601201
- Static ones:
    * Efficient Fluid Simulation on the Surface of a Sphere
    * Huang's bubbles


- Mirela Ben-Chen's geometric flow
https://mirela.net.technion.ac.il/publications/
http://www.cs.technion.ac.il/~mirela/publications/func_thin_films.pdf

- Wen Zheng's levelset bubbles

- Also mention foam (not thin film, but bubbles under water):

- Other thin film papers in computational physics, cite some theoritical ones

######################################
SPH:
- The classical ones (Muller, Babara, etc.)
    https://scholar.google.com/citations?user=RFOOllwAAAAJ&hl=en

- A few SPH papers from Shi-Min Hu (Tao Yang). They did some bubble examples.

- Enriching SPH Simulation by Approximate CapillaryWaves

- Paper from Xiaowei He

- Ando's PIC/FLIP Thin sheet

- Survey:
    https://people.inf.ethz.ch/~sobarbar/papers/Sol14/2014_EG_SPH_STAR.pdf
    (Look at the authors and cite their papers)

- SPH with surface tension:
    There is another survey for this:
    Evaluation of Surface Tension Models for SPH-Based Fluid Animations Using a Benchmark Test

- Akinci


######################################
Point-based surface:
- simulation:
    solving PDEs on point surface (copy some references from Hui's paper)
    different point-base data structures: papers under simplex radar/simplicial particle/must read
- rendering:
    also copy from Hui's papers


#########################################
2D -> Codimension-1
3D -> Codimension-0


